Visual In-Context Prompting

In-context prompting in large language models (LLMs) has become a prevalent approach to improve zero-shot capabilities, but this idea is less explored in the vision domain. Existing visual prompting methods focus on referring segmentation to segment the most relevant object, falling short of addressing many generic vision tasks like open-set segmentation and detection. In this paper, we introduce a universal visual in-context prompting framework for both tasks. In particular, we build on top of an encoder-decoder architecture, and develop a versatile prompt encoder to support a variety of prompts like strokes, boxes, and points. We further enhance it to take an arbitrary number of reference image segments as the context. Our extensive explorations show that the proposed visual in-context prompting elicits extraordinary referring and generic segmentation capabilities to refer and detect, yielding competitive performance to close-set in-domain datasets and showing promising results on many open-set segmentation datasets. By joint training on COCO and SA-1B, our model achieves $57.7$ PQ on COCO and $23.2$ PQ on ADE20K. Code will be available at https://github.com/UX-Decoder/DINOv.

==> resources/table/tab1.tex <==
\begin{table}
  % 表格
  \centering
  \footnotesize
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{lcccc|cccc}
    \toprule
             & \multicolumn{4}{c|}{Referring} & \multicolumn{4}{c}{Generic} \\
             & Text& Image& Visual& In-Context& Text& Image& Visual& In-Context\\
             \midrule
    MQ-Det~\cite{xu2023multi}&   &       &     &      &       \checkmark&       \checkmark&     &      \\
    OWL-VIT~\cite{minderer2022simple}&  &       &     &      &       \checkmark&       \checkmark& &      \\
    GLIP~\cite{li2022grounded}&  &       &  &      &       \checkmark&       &     &      \\
    G-DINO~\cite{liu2023grounding}&    &       &     &      &       \checkmark&       &     &      \\
    OVSeg~\cite{liang2023open}&   \checkmark   &    &     &      &       &     &     &      \\
    SAM~\cite{kirillov2023segment}&  &       &     \checkmark&      &       &  &     &      \\
    SEEM~\cite{zou2023segment}&  \checkmark    &       &     \checkmark    &      \checkmark    &       &  &     &      \\
    SegGPT~\cite{wang2023seggpt}&  &       &     &      \checkmark    &       &  &     &      \checkmark    \\
    Ours&    &    &   \checkmark  &   \checkmark   &  &    &   \checkmark  &     \checkmark  \\
    \bottomrule
    % \label{tab: input output format}
    \end{tabular}
    }
  \caption{\footnotesize A comparison of prompts and tasks of different methods. ``In-Context" denotes visual in-context prompts. Different from previous works, ours is able to perform both referring and generic segmentation with visual prompts and visual in-context prompts. \jianwei{missed some ticks.}
  % \hao{This table might be clearer than Fig.~\ref{fig:scope} but need another figure to illustrate prompt types. You can decide on which to use.}
  }
  \label{tab:prompts and tasks}
  \vspace{-6mm}
\end{table}

==> resources/tex/contrastive_sample.tex <==
\begin{figure*}[t!]
    \centering
    \caption{\ourmodel{} constructs positive and negative samples for generic segmentation and referring segmentation.  }
    \includegraphics[width=0.77\textwidth]{resources/images/contrastive_sample.pdf}
    \vspace{-5pt}
    \label{fig:model_overview}
    % \vspace{-12pt}
\end{figure*}

==> resources/tex/pesudo_code.tex <==
\begin{figure*}[t]
  % Shared Initialization
  \begin{minipage}{\textwidth}
    \begin{algorithm}[H]
      \caption{Pseudo code for \ourmodel{}.}
      \label{alg:shared_initialization}
      \scriptsize
          \Comment{Inputs:~Reference Image($\mathcal{I}$)[B,3,H,W]; Visual Prompt($\mathcal{P}$): Mask\_Prompt[B,N,H,W]; Target Image($\mathbf{I_t}$)}
          \Comment{Variables:~Learnable Queries($Q_s$); Attention Masks between $Q_s$ and $Q_p$(visual prompt features)}
        \Comment{Functions:~Img\_Encoder(),Prompt\_Encoder(),Prompt\_Sample(), Decoder(), MaskHead(), Prompt\_Classifier(), cross\_attn(), output();}
  \Function{init( )}{
     % \var{$Q_o$,$Q_t$,$Q_v$ = $Q_h$.copy()}; \Comment{Initialize object, text, and visual queries.}
     \var{$Q_s$ = $Q_s$.copy()}; \Comment{Initialize segmentation queries.}
     \var{$\mathcal{Z}$ = Img\_Encoder($\mathcal{I}$)}; \Comment{$\mathcal{I}$~and~$\mathcal{Z}$ indicate the reference images and the extracted features.}
     \var{$\mathbf{Z}$ = Img\_Encoder($\mathbf{I_t}$)}; \Comment{$\mathbf{I_t}$~and~$\mathbf{Z}$ indicate the target image ant its extracted features.}
     \var{$\mathcal{F}$ = Prompt\_Encoder($\mathcal{P}, \mathcal{Z}$)}; \Comment{$\mathcal{F}$ denotes all visual prompt features and $\mathcal{P}$ is the input visual prompts.}
     \var{$\mathbf{Q_p}$ = Prompt\_Sample($\mathcal{F}$)}; \Comment{$\mathbf{Q_p}$ denotes the sampled visual prompt features for each semantic category}
     }
  \Function{Prompt\_Sample($\mathcal{F}$)}{
    \STATE \var{$\mathbf{F_{c}}$ = RandomSelect($\mathcal{F}$[$C$], $N$) for $C$ in $\mathcal{F}$}; \Comment{For each semantic category, randomly select $N$ features.}
    \STATE \var{$\mathbf{U_{c}}$ = Average($\mathbf{F_{c}}$)}; \Comment{Perform average aggregation to get unified feature}
     \var{$\mathbf{Q_p}$ = $\{\mathbf{U_0}, ..., \mathbf{U_C}\}$}
     }
  \Function{\ourmodel{}\_Decoder($\mathbf{Q_s}$, $\mathbf{Q_p}$, $\mathbf{Z}$)}{
    \var{$\mathbf{O_s}$ = cross\_attn($\mathbf{Q_s}$, $\mathbf{Z}$)}; \Comment{Cross attend segmentation queries with image features.}
    \var{$\mathbf{O_p}$ = cross\_attn($\mathbf{Q_p}$, $\mathbf{Z}$)}; \Comment{Cross attend sampled visual prompt queries with image features.}
    \var{$\mathbf{M}$, $\mathbf{B}$ = MaskHead($\mathbf{O_s}$)}; \Comment{Get predicted masks $\mathbf{M}$ and boxes $\mathbf{B}$ based on segmentation queries.}
    
    \var{$\mathbf{C_{generic}}$ = PromptClassifier($\mathbf{O_s}$, $\mathbf{O_p}$)};
    
    \var{$\mathbf{C_{refer}}$ = PromptClassifier($\mathbf{O_p}$, $\mathbf{O_s}$)}; 
    
    \Comment{$\mathbf{C_{generic}}$ and $\mathbf{C_{refer}}$ denote to the predict semantic categories depend on the task type.}
      }
  \Function{forward($\mathcal{I}$, $\mathcal{P}$, $\mathbf{I_t}$)}{
     \var{$\mathcal{Z}$, $\mathbf{Z}$, $\mathbf{Q_p}$, $\mathbf{Q_s}$ = init()}; \Comment{Initialization.}
     \For{$i$ in range(max\_iter)}{
    \var{$\mathbf{M}$,$\mathbf{B}$,$\mathbf{C}$ = \ourmodel{}\_Decoder($\mathbf{Z}$, $\mathbf{Q_p}$, $\mathbf{Q_s}$)} \Comment{Decode process.}
     }
  }
  \end{algorithm}
  \end{minipage}
\vspace{-15pt}
\end{figure*}

==> resources/tex/pesudo_code_prompt_sample.tex <==
\begin{figure*}[t]
\vspace{-11pt}
\resizebox{0.999\linewidth}{!}{
  % Shared Initialization
  \begin{minipage}{\textwidth}
    \begin{algorithm}[H]
      \caption{Pseudo code of Prompt Sampling for Generic Segmentation Task.}
      \label{alg:shared_initialization}
      \scriptsize
          \Comment{Inputs:~A list of encoded \textit{reference visual prompt} $\mathcal{F}$ with length $M$, $M$ is the total number of possible prompting examples. The ground-truth semantic category (i.e., dogs) of each reference visual prompt forms another list $\mathcal{C}$ with length $M$. During training, $\mathcal{F}$ is acquired from a batch of training images (i.e., 64 images). During inference, the batch is the whole training image set.}
          \Comment{Variables: Defined maximum in-context length $N$ for each semantic category.}
          \Comment{Output: \textit{Query visual prompt} $Q_p$}
  \Function{Prompt\_Sample($\mathcal{F}$)}{
  \STATE \var{$\textbf{C}$=\textbf{Unique($\mathcal{C}$)}};\Comment{\textbf{$C$} is a list that contains all the semantic categories in this training batch.}
  \STATE \var{$\mathbf{F_{c}}$=\textbf{Dict()}};\Comment{$\mathbf{F_{c}}$ is visual prompt dict, where key is the semantic category and value are the reference prompt features.}
  \STATE \var{$\mathbf{F_{c}}$[c]=[] for $c$ in $\textbf{C}$}; \Comment{Initialize visual prompt dict by semantic category.}
  \STATE \var{$\mathbf{F_{c}}$[c].append(f) for $c$, $f$ in zip($\mathcal{C}$, $\mathcal{F}$)}; \Comment{Gather visual prompts of the same semantic category.}
  \STATE \var{$n = \textbf{Randint(1, $N$}$}; \Comment{Randomly select the number of in-context examples.}
    \STATE \var{$\mathbf{S_{c}}$ = \textbf{RandomSelect}($\mathcal{F}$[$c$], $n$) for $c$ in $\textbf{C}$}; \Comment{For each semantic category, randomly select $n$ prompts to represent a semantic category.}
    \STATE \var{$\mathbf{Q_p}$ = [\textbf{Aggregate}($\mathbf{S_{c}}[c]$) for $c$ in $\textbf{C}$]}; \Comment{Perform prompt aggregation to get one reference prompt token from multiple in-context prompt features for each semantic category.}
     % \var{$\mathbf{Q_p}$ = $[\mathbf{U_0}, ..., \mathbf{U_C}]$}
     }

  \end{algorithm}
  \end{minipage}
\vspace{-35pt}
}
\end{figure*}

==> resources/tex/teaser_fig.tex <==
\begin{figure*}[t!]
    \centering
    \caption{\ourmodel{} is a universal segmentation framework that can do generic segmentation and referring image segmentation. The vision encoder is used to extract image features.  }
    \includegraphics[width=\textwidth]{resources/images/teaser.pdf}
    % \includegraphics[width=0.87\textwidth]{latex/resources/images/main_framework.pdf}
    \vspace{-5pt}
    \label{fig:framework_all}
    % \vspace{-12pt}
\end{figure*}
